DiffusionLight: Light Probes for Free by Painting a Chrome Ball

We present a simple yet effective technique to estimate lighting in a single input image. Current techniques rely heavily on HDR panorama datasets to train neural networks to regress an input with limited field-of-view to a full environment map. However, these approaches often struggle with real-world, uncontrolled settings due to the limited diversity and size of their datasets. To address this problem, we leverage diffusion models trained on billions of standard images to render a chrome ball into the input image. Despite its simplicity, this task remains challenging: the diffusion models often insert incorrect or inconsistent objects and cannot readily generate images in HDR format. Our research uncovers a surprising relationship between the appearance of chrome balls and the initial diffusion noise map, which we utilize to consistently generate high-quality chrome balls. We further fine-tune an LDR diffusion model (Stable Diffusion XL) with LoRA, enabling it to perform exposure bracketing for HDR light estimation. Our method produces convincing light estimates across diverse settings and demonstrates superior generalization to in-the-wild scenarios.

==> 03_method_legacy.tex <==
\iffalse
Note for the tip.
1. explain what the technical problem, how it's challenging  it has to be something that is not obvious to solve
2. Summarize the challenges into short sentences Do the same with solutions. can't explain the challenges and solutions in one or few sentences, it's probably not high-level enough

Outline:
3.1 Prelimnary 
3.2 Inpainting Chromeball
3.3 ControlNet Depth
3.4 The Median ball of Random seed 
3.5 Lora-turing the ball
- Lack of HDR for down stream tasks 
3.5.1 "Black dark prompt"


\fi
\section{Approach}

\subsection{Preliminaries}
% OpenCLIP-ViT/G and CLIP-ViT/L
% https://github.com/mlfoundations/open_clip/blob/91923dfc376afb9d44577a0c9bd0930389349438/src/open_clip/transformer.py#L565

\tanx{
Diffusion models \cite{ho2020denoising} belong to a new family of generative models that model a mapping function between two data distributions by learning the underlying Gaussian Markov process. Let $z_t$ denotes the random variable at $t$-th timestep, the forward diffusion process is defined as $q(z_t | z_{t-1}) = \mathcal{N}(\sqrt{\alpha_t} z_{t-1}, (1 - \alpha_t)I)$, where $\alpha_t$ controls the noise level. By leveraging a property of Gaussian distribution, we can express $z_t$ as:
}
\begin{equation}
    z_t = \sqrt{\bar{\alpha}_t} z_0 + \sqrt{1 - \bar{\alpha}_t} \epsilon, ~ \text{where} ~ \epsilon \sim \mathcal{N}(0, I).
\end{equation}
where $\bar{\alpha}= \prod_{i=1}^{t} \alpha_i$. Thus, we can sample from the target distribution if we can construct a model to reverse this process.



\subsection{Light estimation by synthesizing a chrome ball into the scene}

\pure{Outline:
1. Expected the inpainting model good. (but it didn't) we will fix that}

%\pure{We propose inpainting the chrome ball into the image. We expected that a good inpainting algorithm could blend the ball into the surrounding object/background.}


\label{sec:method_chromeball}

\textbf{Inpainting with Stable Diffusion \& ControlNet} \label{sec:sdxl_controlnet}

\pure{Outline: 1. We fixed it by do a depth control and editing the depth to add the ball}



\iffalse
% บอกว่าวิธีการปัจจุบันเทรนด้วยการ random crop ไม่ใช่เทรนเพื่อเติม object ทำให้ในบางครั้งในการรัน ตัว network เลือกจะเติมส่วนที่หายไปจากภาพ โดยการ
% เราจึงพยายามก้าวข้ามปัญหานี้โดยการใช้ Controlnet-depth เพราะ controlnet ถูกเทรนมาเพื่อบังคับให้ภาพที่ทำการสร้างออกมามี depth เหมือนกับที่ได้ condition เข้าไป โดยเราจะนำการภาพที่ต้องการจะเพิ่มลูกบอกล ไปใส่ยัง off-the-shelf depth prediction network. ซึ่งในงานนี้เราจะใช้ Dense Prediction Transformer (Intel-DPT) เมื่อได้ depth ดังกล่าวจะทำการแก้ไข depth บริเวณที่ต้องการเติมลูกบอลให้เป็น depth ของลูกบอลแทน ด้วยวิธีนี้จะทำให้โอกาส สำเร็จในการเติมลูกบอลสูงขึ้น ซึ่งตัว Controlnet-depth นี้มี publicly avalible pertrain model สำหรับ Stable diffusion หลายเวอร์ชั่น เราได้เลือก stable diffusion XL เนื่องจากภาพลูกบอลที่ได้ออกมาส่วนใหญ่จะเป็นลักษณะ mirror chromeball มากกว่า glossy chromeball
\fi

%\pure{We propose to add a chrome ball to the scene using a recent inpainting method, either text-driven (such as DALL-E, Stable Diffusion, or Blend Diffusion) or image-driven (such as Paint-by-Example). However, the latter may fail because it is trained using random crops of images, which can lead the model to fill in the missing part instead of the chrome ball.}

%\pure{One effective method to encourage a diffusion method to output a chrome ball is to use a ControlNet-depth model. ControlNet-depth is trained to encourage the diffusion output to have the same depth as the given depth input condition. We obtain this depth input using an off-the-shelf depth prediction model called Dense Prediction Transformer (Intel-DPT). We then edit this depth to specify a location to insert the chrome ball. With this method, we achieved a higher success rate in inpainting the chrome ball. ControlNet-depth is publicly available for multiple Stable Diffusion models. We chose Stable Diffusion XL and its corresponding ControlNet-depth model in our method because it is more likely to inpaint mirror chrome balls, while the other variant, Stable Diffusion 1.5, is more likely to paint glossy balls.}


\textbf{The Median ball of Random seed}

\iffalse
%  อย่างไรก็ตามเราพบกว่า seed มีผลกรนะทบเป็นอย่างมากต่อการ inpainting ดังที่แสดงให้เห็นในภาพที \ref{} เราจึงได้ทำการ inpaint ภาพลูกบอลออกมาเป็นจำนวนมาก พบว่า seed ในส่วนใหญ่จะมีแสงชี้ไปในทิศทางเดียวกัน แม้จะมีบาง seed ที่แสงชี้ไปผิดทิศทาง เราจึงปัญหานี้ด้วยการสร้างภาพ ด้วย seed จำนวน N ภาพ จากนั้นนำภาพที่ได้มาทำการหา median ของแต่ละพิกเซลในภาพเพื่อนำ outlier ออกไปจาก โดยภาพที่จะได้จะมีทิศทางถูก แต่มีรายละเอียดที่เป็นลักษณะเบลอ จึงทำการนำภาพเบลอดังกล่าวไปใส่ noise และทำการเริ่ม inpaint ใหม่อีกครั้ง โดยจะทำซ้ำแบบนี้ N_k รอบ เพื่อให้ได้ภาพบอลที่ดีที่สุดเพียง 1 ลูกต่อภาพ
\fi

%\pure{However, we found that the random seed had a significant impact on the inpainting result. Some seeds generated chrome balls with invalid light directions. To address this problem, we generated chrome balls from $N$ random seeds and then finding the median for each pixel of the chrome balls to remove outliers. This step created a blurry chrome ball image due to the high difference in the detail of the scene shown in chrome balls. However, This median chromeball does have correct lighting direction. We then added random noise to this median ball to obtain the initial noise for the inpainting step. We repeated this step $N_k$ times to obtain a good median chrome ball, which we then used as the initial chrome ball for one final inpainting step.}

\tanx{
We analyze the effects of the initial latent code $z_t$ on the appearance of the generated chrome balls $x_0$ by inpainting a chrome ball with a radius $r = 256$ pixels at the center of images using the pipeline described in Section \ref{sec:sdxl_controlnet}. Figure \ref{fig:noise_appearance_relationship} suggests that 
}

\input{figs/noise_appearance_relationship_rev1}

\textbf{LoRA fine-tuning on the ball}

\tanx{
While the median algorithm has shown satisfactory performance, the computational cost remains relatively high. This is because a sufficiently large number of balls must be generated per iteration to obtain a representative average ball given the existence of \textit{inferior} initial latent code $z_t$. To address this issue, we propose to fine-tune the diffusion model to guide the denoising process towards \textit{good} chrome balls. 

% Specificially, we train a LoRA on 1412 LDRs generated using Text2Light \cite{chen2022text2light} and their corresponding chrome balls.
}

\tanx{
More formally, let $z_0$ be a latent representation of a $1024 \times 1024$ scene image with the corresponding ground-truth chrome ball with radius $r = 256$ placed at the center. The training objective can be described as:
}
\begin{equation}
    placeholder
\end{equation}

\pure{\todomark Said about with context training}

\textbf{Getting HDR output from Model that output LDR}


\iffalse
%  อย่างไรก็ตาม ภาพที่ได้ออกมาจากการ inpaint ลูกบอลเป็นภาพ LDR (Low dynamic range) ซึ่งไม่เหมาะกับการนำไปใช้งานต่อใน object insertion / relighting task. เราจึงได้เสนอวิธีการนำภาพแบบ HDR (High Dynamic range) กลับมาจาก LDR โดยการใช้ bracket of exposure. ซึ่งเราจะสามารถสามารถควบคุมการทำให้ภาพมืดลงได้ โดยการใส่ข้อความ "black dark" ลงไปใน prompt อย่างไรก็ตามภาพที่ได้ออกมานั้น มีความสว่างที่ต่างกันออก ทำให้เราไม่สามารถควบคุมค่า exposure value เพื่อทำการ reconstruct HDR กลับออกมาได้ เราจึงได้ทำการ finetune with LORA โดยใช้สร้างภาพที่ปกติ (มีค่า EV0) และภาพที่มืดลง (มีค่า EV -ev) ด้วย HDR text2light ทั้งสิ้น 1000 ภาพเพื่อเทรนภาพทีมีลักษณะปกติ  และภาพที่มืดกว่าที่ทราบค่า EV แน่นอน 
% ใช้การ detail จากภาพปกติ แต่ใช้ luminance จากทั้งภาพปกติและภาพภาพที่มืดกว่าโดยการแปลงภาพจาก RGB space เป็น XYZ space เพื่อให้ได้ Luminace (Y) ออกมา จากนั้นจะทำการรวมค่า Luminance ใหม่โดย สมการ \ref{ใส่สมการ} เมื่อได้ luminace ที่รวมกันของทั้งสองภาพแล้ว ไม่สามารถนำไปอัปเดตค่าสีใน XYZ space แต่เนื่องจากการเปลี่ยนค่า luminance จะส่งผลกระทบต่อสีในภาพเป็นอย่างมาก เราจึงทำการเปลี่ยนจาก Luminance เป็น perceptive luminace (L*) ใน L*a*b* colorspace เพื่อมารวมกับ a*b* ที่ได้จากภาพปกติ (EV0) ซึ่งสามารถนำมารวมกับแปลงกับเป็นภาพ HDR ใน RGB colorspace สำหรับใช้งานในลำดับต่อไปไดก้
\fi

%\pure{The off-the-shelf diffusion model we are using outputs a low-dynamic range (LDR) image, which has limited capacity for downstream tasks such as relighting for 3D object insertion. Therefore, we propose to obtain a high-dynamic range (HDR) image using the bracket exposure method. We can generate a chrome ball with a lower exposure value by adding "black dark" to the prompt, but this method does not yield the exact exposure value. To overcome this problem, we will fine-tune the LoRA model to predict the exact exposure value.}

\pure{\todomark explain Text2light Lora training}

\pure{\todomark explain that we handing the different detail in the scene by merging only the luminance}



%\subsection{Direct light estimation without synthesizing a chrome ball}



==> 05_limitations.tex <==
\section{Limitations}

\pure{We assume orthographic.} Additionally, while our approach outperforms state-of-the-art methods, the computational cost remains relatively high due to the slow sampling speed of diffusion models. 
We believe that further improvements can be achieved with marginal performance degradation by employing more sampling-efficient models such as InstaFlow \cite{}.

% Although addressing this issue is outside the scope of our work, we believe that further improvements can be achieved with marginal performance degradation by employing more sampling-efficient models such as InstaFlow \cite{}. 


% through designing a discriminative model based on diffusion

% - Orthographic camera

% - relatively slow inference speed (compared to existing methods). However, works on diffusion sampling acceleration can address it with marginal performance degradation (e.g. InstaFlow, progressive distillation)

==> figs/aba_lightinfo_darkcomposite.tex <==
% z1 = seed 140
% z2 = seed 150
% z3 = seed 147

\tabulinesep=0.1pt
\begin{figure}
    \centering

    \begin{tabu} to \textwidth {
        @{}
        % 1st example
        c@{\hspace{3pt}}
        c@{\hspace{0.5pt}}
        c@{\hspace{0.5pt}}
        c@{\hspace{0.5pt}}
        c@{\hspace{0.5pt}}
        c@{\hspace{0.5pt}}
        c@{}
    }

        \multicolumn{1}{c}{\shortstack{\scriptsize Input}} & 
        \multicolumn{1}{c}{\shortstack{\scriptsize Pred\#1}} &
        \multicolumn{1}{c}{\shortstack{\scriptsize Pred\#2}} & 
        \multicolumn{1}{c}{\shortstack{\scriptsize Pred\#3}} & 
        \multicolumn{1}{c}{\shortstack{\scriptsize Pred\#4}} &
        \multicolumn{1}{c}{\shortstack{\scriptsize Pred\#5}}
        \\
        
        % input
        \multirow{3}{*}{\noindent\parbox[c]{0.145\textwidth}{\includegraphics[width=0.145\textwidth]{storage/aba_lightinfo_darkcomposite/input/dark_car.pdf}}} &
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/normal/car_variation0.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/normal/car_variation1.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/normal/car_variation2.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/normal/car_variation3.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/normal/car_variation4.pdf}}
        
        \\

        &
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark/car_variation0.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark/car_variation1.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark/car_variation2.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark/car_variation3.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark/car_variation4.pdf}}
        
        \\

        &
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark_08/car_variation0.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark_08/car_variation1.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark_08/car_variation2.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark_08/car_variation3.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark_08/car_variation4.pdf}}
        
        \\

        \thickhline

        % input
        \multirow{3}{*}{\noindent\parbox[c]{0.145\textwidth}{\includegraphics[width=0.145\textwidth]{storage/aba_lightinfo_darkcomposite/input/dark_cat.pdf}}} &
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/normal/cat_variation0.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/normal/cat_variation1.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/normal/cat_variation2.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/normal/cat_variation3.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/normal/cat_variation4.pdf}}
        
        \\

        &
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark/cat_variation0.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark/cat_variation1.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark/cat_variation2.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark/cat_variation3.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark/cat_variation4.pdf}}
        
        \\

        &
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark_08/cat_variation0.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark_08/cat_variation1.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark_08/cat_variation2.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark_08/cat_variation3.pdf}} & 
        \noindent\parbox[c]{0.063\textwidth}{\includegraphics[width=0.063\textwidth]{storage/aba_lightinfo_darkcomposite/dark_08/cat_variation4.pdf}}
        
        \\
        
    \end{tabu}

    %\caption{Comparison of chrome balls generated with the \textit{normal} prompt using different denoising strengths: 1.0 (1\textsuperscript{st} row), 0.9 (1\textsuperscript{st} row), and 0.8 (1\textsuperscript{st} row). \todo{fix caption}}

    % exposure compensation value
    \caption{Luminance is determined in the first few steps of the denoising process. Given an input image composited with the ball generated from the ``black dark'' prompt, we apply SDEdit \cite{meng2022sdedit} by adding noise to $\vect{z}_T$ to simulate the diffusion process up to time step $\gamma t$, where $0 < \gamma \leq 1$. For each input image, we show results generated with the regular prompt using different values of $\gamma$: 1.0 (1\textsuperscript{st} row), 0.9 (2\textsuperscript{nd} row), and 0.8 (3\textsuperscript{rd} row). The chrome balls are visibly darker when using $\gamma < 1$ because the light bias from the dark ball in the input influences the sampling process.}
    
    % reverse the diffusion  process into the noise at $\vect{x}_{1000}$, $\vect{x}_{900}$ and, $\vect{x}_{800}$} and do a diffusion process using regular prompt shown in a consecutive row. $\vect{x}_{900}$ and, $\vect{x}_{800}$} still has the effect of a "black dark" ball which is noticeable darker.
    
    
    \label{fig:aba_lightinfo_darkcomposite}
\end{figure}

% previous = 0.084

==> figs/additional_object_insertion_halfpage.tex <==
% ==============================
% Additional Result for object insertion
% ===============================

\tabulinesep=0.5pt
\begin{figure*}[!t]
    \centering

    \begin{tabu} to \textwidth {
        @{}
        % 1st example
        c@{\hspace{2pt}}
        c@{\hspace{2pt}}
    }

        \multicolumn{1}{c}{\shortstack{ Input object}}
        &
        \multicolumn{1}{c}{\shortstack{Input object}} \\
        \noindent\parbox[c]{0.5\textwidth}{\centering\includegraphics[height=0.2\textwidth]{storage/appendix_object_insertion/input_bag.pdf}} &
        \noindent\parbox[c]{0.5\textwidth}{\centering\includegraphics[height=0.2\textwidth]{storage/appendix_object_insertion/input_shoe.pdf}}
    \end{tabu}

    \begin{tabu} to \textwidth {
        @{}
        % 1st example
        c@{\hspace{2pt}}
        c@{\hspace{2pt}}
        c@{\hspace{2pt}}
        c@{\hspace{2pt}}
    }

        \multicolumn{1}{c}{\shortstack{ Before relighting}}
        &
        \multicolumn{1}{c}{\shortstack{ After relighting}}
        &
        \multicolumn{1}{c}{\shortstack{ Before relighting}}
        &
        \multicolumn{1}{c}{\shortstack{ After relighting}}
        \\ 
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/bedzoom_bag_no_light.pdf}} &
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/bedzoom_bag.pdf}}&
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/bedzoom_shoe_no_light.pdf}} &
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/bedzoom_shoe.pdf}}
        % bag
        \\
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/cambodia2tilt_bag_nolight.pdf}} &
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/cambodia2tilt_bag.pdf}} &
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/cambodia2tilt_shoe_nolight.pdf}} &
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/cambodia2tilt_shoe.pdf}}
    \end{tabu}
    \caption{
    We synthetically render each 3D object into input images using our estimated lighting.
    %results for virtual object insertion.
    }
    \label{fig:additional_object_insertion}
\end{figure*}

==> figs/compare_distribution_median.tex <==
% z1 = seed 140
% z2 = seed 150
% z3 = seed 147

\tabulinesep=2pt
\begin{figure}
    \centering

    \begin{tabu} to \textwidth {
        @{}
        c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        c@{}
    }
        
        % input
        \noindent\parbox[c]{0.09\textwidth}{\includegraphics[width=0.09\textwidth]{storage/compare_distribution_median/paper_distribution_car_input.pdf}} 
        &
        \noindent\parbox[c]{0.38\textwidth}{\includegraphics[width=0.38\textwidth]{storage/compare_distribution_median/paper_distribution_car_it0.pdf}} 
        \\

        \hline

        \noindent\parbox[c]{0.09\textwidth}{\shortstack{\scriptsize Median ball \\ \includegraphics[width=0.09\textwidth]{storage/compare_distribution_median/paper_distribution_car_median.pdf}}}
        
        
        % {\centering \scriptsize Median ball} \\ \includegraphics[width=0.09\textwidth]{storage/compare_distribution_median/paper_distribution_car_median.pdf}} 
        &
        \noindent\parbox[c]{0.38\textwidth}{\includegraphics[width=0.38\textwidth]{storage/compare_distribution_median/paper_distribution_car_it1.pdf}} 
        \\
        
    \end{tabu}

    \caption{Compare median distribution. \tanx{placeholder}}
    \label{fig:compare_median_distribution}
\end{figure}

==> figs/noise_appearance_relationship_rev1.tex <==
% z1 = seed 140
% z2 = seed 150
% z3 = seed 147

\tabulinesep=0.5pt
\begin{figure}
    \centering

    \begin{tabu} to \textwidth {
        @{}
        % 1st example
        c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        % c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        % c@{\hspace{1pt}}
        c@{}
    }
        
        % input
        \noindent\parbox[c]{0.090\textwidth}{\includegraphics[width=0.090\textwidth]{storage/noise_appearance_relationship_whiteBG/input/airport_seed150.pdf}} & 
        \noindent\parbox[c]{0.090\textwidth}{\includegraphics[width=0.090\textwidth]{storage/noise_appearance_relationship_whiteBG/input/castle3_seed150.pdf}} & 
        \noindent\parbox[c]{0.090\textwidth}{\includegraphics[width=0.090\textwidth]{storage/noise_appearance_relationship_whiteBG/input/panda_seed150.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship/input/house_seed150.pdf}} &
        \noindent\parbox[c]{0.090\textwidth}{\includegraphics[width=0.090\textwidth]{storage/noise_appearance_relationship_whiteBG/input/street2_seed150.pdf}} & 
        \noindent\parbox[c]{0.090\textwidth}{\includegraphics[width=0.090\textwidth]{storage/noise_appearance_relationship_whiteBG/input/opera_house_seed150.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/input/slum_seed150.pdf}} &

        \\

        % seed 150
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/airport_seed150.pdf}} & 
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/castle3_seed150.pdf}} & 
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/panda_seed150.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/house_seed150.pdf}} &
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/street2_seed150.pdf}} & 
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/opera_house_seed150.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/slum_seed150.pdf}} &
        
        \\

        % seed 150
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/airport_seed150.pdf}} & 
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/castle3_seed150.pdf}} & 
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/panda_seed150.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/house_seed150.pdf}} &
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/street2_seed150.pdf}} & 
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/opera_house_seed150.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/150/slum_seed150.pdf}} &
        
        \\

        % seed 147
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/147/airport_seed147.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/147/castle3_seed147.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/147/panda_seed147.pdf}} & 
        % % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/147/house_seed147.pdf}} &
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/147/street2_seed147.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/147/opera_house_seed147.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/147/slum_seed147.pdf}} &

        % \\

        % seed 140
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/37/airport_seed37.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/37/castle3_seed37.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/37/panda_seed37.pdf}} & 
        % % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/140/house_seed140.pdf}} &
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/37/street2_seed37.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/37/opera_house_seed37.pdf}} & 
        % % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/140/slum_seed140.pdf}} &

        % \\ 
        
        \arrayrulecolor{red}\hline

        % seed 140
        \multicolumn{1}{|c}{\noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/median_lora/airport_ev-00_seed140.pdf}}} & 
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/median_lora/castle3_ev-00_seed140.pdf}} & 
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/median_lora/panda_ev-00_seed140.pdf}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/median_lora/house_seed140.pdf}} &
        \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/median_lora/street2_ev-00_seed140.pdf}} & 
        \multicolumn{1}{c|}{\noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/median_lora/opera_house_ev-00_seed140.pdf}}} & 
        % \noindent\parbox[c]{0.075\textwidth}{\includegraphics[width=0.075\textwidth]{storage/noise_appearance_relationship_whiteBG/median_lora/slum_ev-00_seed140.pdf}} &

        \\ \arrayrulecolor{red}\hline
        \arrayrulecolor{black}
        
    \end{tabu}

    \caption{We observed that the initial noise map encodes some semantic information and patterns. There is a certain initial noise map that consistently produces a disco chrome ball across input images, as shown in the second row. The last row shows our results on these input images.
    %Relationship between initial noise map and appearance of chrome balls. The 2\textsuperscript{nd} row shows results when inpainting input images (1\textsuperscript{st} row) using a ``disco'' noise map while the 3\textsuperscript{rd} is generated using our proposed method. Prompt: ``a chrome ball''
    }

    % \caption{Relationship between initial noise map $\vect{z}_T$ and appearance of chrome balls. The first row shows the input images. The 2nd - 3rd rows contain results when starts sampling from different $\vect{z}_T$. The last row is generated using our proposed pipeline. Prompt: ``a chrome ball''}

    % \caption{Relationship between initial noise map $\vect{z}_T$ and appearance of chrome balls. The first row shows the input images. The 2nd - 4th rows contain results when starts sampling from different $\vect{z}_T$. The last row is generated using our proposed pipeline. Prompt: ``a chrome ball'' \todo{change to better examples}}

    % \caption{Relationship between initial noise map $\vect{z}_T$ and appearance of chrome balls. The first row shows the input images. The following rows contain results when starts sampling from different $\vect{z}_T$ using UniPC \cite{zhao2023unipc} with 30 steps. Prompt: ``a chrome ball''}
    \label{fig:noise_appearance_relationship}
\end{figure}


% \setlength\tabcolsep{0pt}
% \begin{figure}
%     \centering
%     \begin{tabularx}{\textwidth}{X}
%         \noindent\parbox[c]{\hsize}{
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/airport_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/castle3_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/panda_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/house_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/street2_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/opera_house_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/slum_seed150.pdf}
%         } \\[8pt]

%         \noindent\parbox[c]{\hsize}{
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/airport_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/castle3_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/panda_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/house_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/street2_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/opera_house_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/slum_seed140.pdf}
%         } \\[8pt]

%         \noindent\parbox[c]{\hsize}{
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/airport_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/castle3_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/panda_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/house_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/street2_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/opera_house_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/slum_seed150.pdf}
%         } \\[8pt]

%         \noindent\parbox[c]{\hsize}{
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/airport_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/castle3_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/panda_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/house_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/street2_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/opera_house_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/slum_seed147.pdf}
%         } \\

%     \end{tabularx}
%     \caption{Relationship between initial latent code $z_T$ and generated chrome balls $x_0$. The first row shows the input images. Each row in the 2nd - 4th lines contains results from different $z_T$. Prompt: ``a chrome ball''}
%     \label{fig:noise_appearance_relationship}
% \end{figure}

% \setlength\tabcolsep{3pt}
% \begin{figure}
%     \centering
%     \begin{tabularx}{\textwidth}{lX}

%         \shortstack[l]{\scriptsize Input} & \noindent\parbox[c]{\hsize}{
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/airport_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/castle3_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/panda_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/house_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/library_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/street2_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/restaurant_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/opera_house_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/input/temple_seed150.pdf}
%         } \\[8pt]

%         \shortstack[l]{\scriptsize Noise $z_1$} & \noindent\parbox[c]{\hsize}{
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/airport_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/castle3_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/panda_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/house_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/library_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/street2_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/restaurant_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/opera_house_seed140.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/140/temple_seed140.pdf}
%         } \\[8pt]

%         \shortstack[l]{\scriptsize Noise $z_2$} & \noindent\parbox[c]{\hsize}{
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/airport_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/castle3_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/panda_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/house_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/library_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/street2_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/restaurant_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/opera_house_seed150.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/150/temple_seed150.pdf}
%         } \\[8pt]

%         \shortstack[l]{\scriptsize Noise $z_1$} & \noindent\parbox[c]{\hsize}{
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/airport_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/castle3_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/panda_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/house_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/library_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/street2_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/restaurant_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/opera_house_seed147.pdf}
%             \includegraphics[width=0.13\columnwidth]{storage/noise_appearance_relationship/147/temple_seed147.pdf}
%         } \\

%     \end{tabularx}
%     \caption{xxx}
%     \label{fig:noise_appearance_relationship}
% \end{figure}

==> figs/qualitative_indoor.tex <==
\tabulinesep=0.5pt
\begin{figure}
    \centering

    \begin{tabu} to \textwidth {
        @{}
        % 1st example
        c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        % c@{\hspace{1pt}}
        % c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        c@{}
    }
        %%%%%%%%%%%%%%%%%%%%%
        % 1 LINE
        %%%%%%%%%%%%%%%%%%%%%
        \multicolumn{1}{c}{\shortstack{\tiny Input image}}
        & \multicolumn{1}{c}{\shortstack{\tiny GT}}
        & \multicolumn{1}{c}{\shortstack{\tiny StyleLight \cite{wang2022stylelight}}}
        % & \multicolumn{1}{c}{\shortstack{\tiny Ours (ZS)}}
        & \multicolumn{1}{c}{\shortstack{\tiny Ours (ZS+I)}}
        % & \multicolumn{1}{c}{\shortstack{\tiny Ours (LR)}}
        & \multicolumn{1}{c}{\shortstack{\tiny Ours (LR+I)}} &
        \\

        % input image
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/input/9C4A0205_input.png}} 
        
        % mirror ball
        &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/ball/9C4A0205_gt.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/ball/9C4A0205_stylelight.png}} &  
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/ball/9C4A0205_median.png}} &
       
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/ball/9C4A0205_medianlora.png}} & 
        
        \\

        &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/envmap/9C4A0205_gt.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/envmap/9C4A0205_stylelight.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/envmap/9C4A0205_median.png}} &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/envmap/9C4A0205_medianlora.png}} & 
        \\

        %%%%%%%%%%%%%%%%%%%%%
        % 1 LINE
        %%%%%%%%%%%%%%%%%%%%%

        % input image
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/input/9C4A4427_input.png}} 
        
        % mirror ball
        &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/ball/9C4A4427_gt.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/ball/9C4A4427_stylelight.png}} &  
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/ball/9C4A4427_median.png}} &
       
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/ball/9C4A4427_medianlora.png}} & 
        
        \\

        &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/envmap/9C4A4427_gt.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/envmap/9C4A4427_stylelight.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/envmap/9C4A4427_median.png}} &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/envmap/9C4A4427_medianlora.png}} & 
        \\

        %%%%%%%%%%%%%%%%%%%%%
        % 1 LINE
        %%%%%%%%%%%%%%%%%%%%%

        % input image
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/input/9C4A9174_input.png}} 
        
        % mirror ball
        &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/ball/9C4A9174_gt.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/ball/9C4A9174_stylelight.png}} &  
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/ball/9C4A9174_median.png}} &
       
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/ball/9C4A9174_medianlora.png}} & 
        
        \\

        &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/envmap/9C4A9174_gt.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/envmap/9C4A9174_stylelight.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/envmap/9C4A9174_median.png}} &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/indoor/envmap/9C4A9174_medianlora.png}} & 
        \\

    \end{tabu}
    \caption{
    Qualitative rendering results for Indoor dataset \cite{garder2017lavelindoor} of Stylelight \cite{wang2022stylelight} and different variants of our proposed pipeline (ZS: zero-shot, LR: LoRA, I: iterative). For each input image, we show the rendered mirror sphere (first row) and the predicted environment map (second row) from each method. 
    }
    \label{fig:qualitative_indoor}
\end{figure}

==> figs/qualitative_polyhaven.tex <==
\tabulinesep=0.5pt
\begin{figure}
    \centering

    \begin{tabu} to \textwidth {
        @{}
        % 1st example
        c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        % c@{\hspace{1pt}}
        % c@{\hspace{1pt}}
        c@{\hspace{1pt}}
        c@{}
    }
        %%%%%%%%%%%%%%%%%%%%%
        % 1 LINE
        %%%%%%%%%%%%%%%%%%%%%
        \multicolumn{1}{c}{\shortstack{\tiny Input image}}
        & \multicolumn{1}{c}{\shortstack{\tiny GT}}
        & \multicolumn{1}{c}{\shortstack{\tiny StyleLight \cite{wang2022stylelight}}}
        % & \multicolumn{1}{c}{\shortstack{\tiny Ours (ZS)}}
        & \multicolumn{1}{c}{\shortstack{\tiny Ours (ZS+I)}}
        % & \multicolumn{1}{c}{\shortstack{\tiny Ours (LR)}}
        & \multicolumn{1}{c}{\shortstack{\tiny Ours (LR+I)}} &
        \\

        % input image
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/input/nkuhlu_4k_input.png}} 
        
        % mirror ball
        &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/ball/nkuhlu_4k_gt.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/ball/nkuhlu_4k_stylelight.png}} &  
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/ball/nkuhlu_4k_median.png}} &
       
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/ball/nkuhlu_4k_medianlora.png}} & 
        
        \\

        &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/envmap/nkuhlu_4k_gt.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/envmap/nkuhlu_4k_stylelight.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/envmap/nkuhlu_4k_median.png}} &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/envmap/nkuhlu_4k_medianlora.png}} & 
        \\

        %%%%%%%%%%%%%%%%%%%%%
        % 1 LINE
        %%%%%%%%%%%%%%%%%%%%%

        % input image
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/input/abandoned_greenhouse_4k_input.png}} 
        
        % mirror ball
        &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/ball/abandoned_greenhouse_4k_gt.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/ball/abandoned_greenhouse_4k_stylelight.png}} &  
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/ball/abandoned_greenhouse_4k_median.png}} &
       
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/ball/abandoned_greenhouse_4k_medianlora.png}} & 
        
        \\

        &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/envmap/abandoned_greenhouse_4k_gt.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/envmap/abandoned_greenhouse_4k_stylelight.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/envmap/abandoned_greenhouse_4k_median.png}} &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/envmap/abandoned_greenhouse_4k_medianlora.png}} & 
        \\

        %%%%%%%%%%%%%%%%%%%%%
        % 1 LINE
        %%%%%%%%%%%%%%%%%%%%%

        % input image
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/input/hotel_room_4k_input.png}} 
        
        % mirror ball
        &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/ball/hotel_room_4k_gt.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/ball/hotel_room_4k_stylelight.png}} &  
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/ball/hotel_room_4k_median.png}} &
       
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/ball/hotel_room_4k_medianlora.png}} & 
        
        \\

        &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/envmap/hotel_room_4k_gt.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/envmap/hotel_room_4k_stylelight.png}} & 
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/envmap/hotel_room_4k_median.png}} &
        \noindent\parbox[c]{0.080\textwidth}{\includegraphics[width=0.080\textwidth]{storage/ball_env/polyhaven/envmap/hotel_room_4k_medianlora.png}} & 
        \\

    \end{tabu}
    \caption{
    Qualitative rendering results for Poly Haven dataset of Stylelight \cite{wang2022stylelight} and different variants of our proposed pipeline (ZS: zero-shot, LR: LoRA, I: iterative). For each input image, we show the rendered mirror sphere (first row) and the predicted environment map (second row) from each method. 
    }
    \label{fig:qualitative_polyhaven}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

